A phase transition between positional and semantic learning in a solvable model of dot-product attention

Many empirical studies have provided evidence for the emergence of algorithmic mechanisms (abilities) in the learning of language models, that lead to qualitative improvements of the model capabilities. Yet, a theoretical characterization of how such mechanisms emerge remains elusive. In this paper, we take a step in this direction by providing a tight theoretical analysis of the emergence of semantic attention in a solvable model of dot-product attention. More precisely, we consider a non-linear self-attention layer with trainable tied and low-rank query and key matrices. In the asymptotic limit of high-dimensional data and a comparably large number of training samples we provide a tight closed-form characterization of the global minimum of the non-convex empirical loss landscape. We show that this minimum corresponds to either a positional attention mechanism (with tokens attending to each other based on their respective positions) or a semantic attention mechanism (with tokens attending to each other based on their meaning), and evidence an emergent phase transition from the former to the latter with increasing sample complexity. Finally, we compare the dot-product attention layer to a linear positional baseline, and show that it outperforms the latter using the semantic mechanism provided it has access to sufficient data.

==> Appendices/A.tex <==
\subsection{Empirical scaling of \texorpdfstring{$\alpha=d/n$}{alpha=d/n}}\label{app:sec:scaling}
In the following we verify that our experiments are consistent with the scaling behaviour predicted from the theory.
We jointly increase $d$ and $n$ for a fixed value of $\alpha$.
In Fig.~\ref{fig:scaling-n-d-1} we indeed observe the expected behaviour for an exemplary value of $\alpha=2$.
The same holds for the summary statistics $\theta$ and $m$, which concentrate as $d$ and $n$ jointly grow, shown in Fig.~\ref{fig:sem-pos-crossover-phase-diagram} (left) in the main text.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/d_scaling_omega_0.3.pdf}
    \caption{Scaling $d$ and $n$ jointly for $\alpha=1.5$ approaches the theoretical prediction of the generalization error of the positional and semantic local minima. Experimental settings as in Fig.~\ref{fig:free-entropy-crossover-omega0.3}, with 70 runs per datapoint.}
\label{fig:scaling-n-d-1}
\end{figure}




\subsection{Alternative hyperparameters}

We provide supplementary results for different parameter settings.
Fig.~\ref{fig:supplemental-settings} on the left shows more slices from the phase diagram that appears in the main Fig.~\ref{fig:sem-pos-crossover-phase-diagram}.
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.3\textwidth]{figures/omega_slices.pdf}
    \includegraphics[width=0.3\textwidth]{figures/lmbda_slices.pdf}
    \includegraphics[width=0.3\textwidth]{figures/sigma_slices.pdf}
\caption{ \textit{Alternative Parameters.} Mixed positional/semantic teacher for $\omega=0.3$. Settings is $r_s=r_t=1,L=2, A=((0.6,0.4),(0.4,0.6)),\cov_1=\cov_2=0.25 \mathbb{I}_d$, $\emb_1=\mathbf{1}_d=-\emb_2$ and $\Qstar\sim\mathcal{N}(0,\mathbb{I}_d)$. While keeping all other settings the same, we vary from left to right: The target positionality $\omega$, the student regularizer $\lambda$ and the standard deviation $\sigma$ (which is $0.5 = \sqrt{\cov_1}$) . Experiment settings as in Fig.~\ref{fig:free-entropy-crossover-omega0.3}.
    }
    \label{fig:supplemental-settings}
\end{figure}
For the experimental section of the main text, we chose a specific $A$ for definiteness.
In the following, we present the same results for a different $A$ with a stronger off-diagonal and a higher rank,
\begin{align}
    \label{eq:other_A}
    A=\begin{pmatrix}
        0.3&0.7\\
        0.8&0.2
    \end{pmatrix}.
\end{align}
In Fig.~\ref{fig:another-A-PD} we present the analogous simulations to  Fig.~\ref{fig:sem-pos-crossover-phase-diagram} (center, right).
While the global phenomena match the previous example, the details of the transitions location differ.
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/attention_train_error_pdotherA.pdf}
    
    \caption{\textit{Alternative Positional Matrix.} $r_s=r_t=1,L=2, \cov_1=\cov_2=0.25 \mathbb{I}_d$, $\emb_1=-\emb_2$ and $\emb_1,\Qstar\sim\mathcal{N}(0,\mathbb{I}_d)$  independently. Here, we use a definite matrix $A$ from \eqref{eq:other_A} , which differs form the one used in the main text. Experiments were conducted as in Fig.~\ref{fig:free-entropy-crossover-omega0.3}.}
    \label{fig:another-A-PD}
\end{figure}


\subsection{Uninformed initialization and training via Adam}\label{app:sec:random}

In or experiments, to obtain the empirical results, we initialize the GD optimizer in an informed fashion, i.e. initializing $\Qstar$ of the student with $r=1$  as either $\emb_1$ (positional) or $\Qstar$ (semantics). 
GD then converges in the two local optima described by our theory.

Since our theory only ascertains that these solutions predicted are indeed fixed points of GD for large sizes, this does not have direct implications for other types of optimization algorithms.
In Fig.~\ref{fig:GD-comparison} we show that indeed running the Adam optimizer from an \textit{uninformed} initialization may lead one to either of the local minima for $d=100$.
For larger $d$ we observe the semantic minimum is reached less often than the positional minimum, and a considerable number of times the algorithm simply does not find either of them.

\begin{figure}[ht]
    \centering
\includegraphics[width=0.4\textwidth]{figures/init-vary-2.pdf}
\includegraphics[width=0.4\textwidth]{figures/init-vary-1.pdf}
    \caption{\textit{Comparing GD and Adam.} Settings as in Fig.~\ref{fig:free-entropy-crossover-omega0.3} for the sample complexity $\alpha = 2$. The student parameter $\mathbf{Q}$ is obtained via either \textbf{(left)} positional and semantic informed initialization and \textbf{(right)} GD training from a random initialization are compared. Each point represents a single run. For the informed GD, we used the same optimization parameters as in Fig.~\ref{fig:free-entropy-crossover-omega0.3} (24 runs per initialization). For Adam we trained on the same data, but for $2,500$ epochs with learning rate $\eta=0.01$ (showing 140 runs). }
    \label{fig:GD-comparison}
\end{figure}


